SpecEval: Evaluating Code Comprehension in Large Language Models via Program Specifications

Large Language models have achieved impressive performance in automated software engineering. Extensive efforts have been made to evaluate the abilities of code LLMs in various aspects, with an increasing number of benchmarks and evaluation frameworks proposed. Apart from the most sought-after capability of code generation, the capability of code comprehension is being granted growing attention. Nevertheless, existing works assessing the code comprehension capability of LLMs exhibit varied limitations. Evaluation frameworks like CRUXEval and REval usually focus on code reasoning tasks over a certain input case, leading to a limited range of execution traces covered, resulting in a loss in code semantics examined and the inability to assess the comprehensive understanding of LLMs concerning the target program. To tackle these challenges, we propose SpecEval, a novel black-box evaluation framework to evaluate code comprehension in LLMs via program specifications. Inspired by the idea that specifications can act as a comprehensive articulation of program behaviors concerning all possible execution traces, we employ formalized program specifications to represent program semantics and perform comprehensive evaluations. In particular, four specification-related tasks are designed meticulously to assess the capability of LLMs from basic to advanced levels. Counterfactual analysis is further conducted to study the performance variance of LLMs under semantics-preserving perturbations. Systematic experiments are conducted on six state-of-the-art LLMs. Extensive experimental results present a below-satisfactory performance of LLMs on specification-related tasks, revealing the limitations of existing LLMs in terms of articulating program semantics with formal specifications. Counterfactual analysis also reveals the sensitivity of LLMs towards semantic-preserving perturbations.

==> sections/preliminary.tex <==
\section{Preliminary Definitions} \label{sec:preliminary}

In this section, we aim to present the definitions for several abstract concepts that will be frequently discussed later in this paper, in order to facilitate the descriptions hereinafter.

\subsubsection{Program States}
For the first concept, program state, we take the view of operational semantics~\cite{plotkin1981structural} and regard program state as the set of values for all variables involved in the program. Formally, the concept can be defined as follows.

\begin{definition}[Program states]
A program state is a mapping $\sigma: X \rightarrow V$, where $X$ is the set of all program variables and $V$ denotes the space of all possible variable values.
\end{definition}

\subsubsection{Program Specifications}
Specifications describe certain constraints on all program states $\sigma \in \Sigma$ that it covers (depending on its position and scope), where $\Sigma$ denotes the set of all program states covered. Consider such a specification expressed in first-order logic expression on program variables, such as $x == y + z$, the constraint it describes actually constitutes a boolean function $f: \Sigma \rightarrow \{true,false\}$. In the instance mentioned above, $f$ is a boolean function mapping the values of $x$, $y$, and $z$ to $\{true, false\}$, depending on whether the value of $x$ equals $y+z$ or not. Based on these insights, specifications can be formally defined as follows.

\begin{definition}[Program specifications]
A specification $s$ is a 2-tuple $(\Sigma, f)$, where $\Sigma$ is the set of all program states covered by the specification and $f: \Sigma \rightarrow \{true,false\}$ is a boolean function.
\end{definition}

\subsubsection{Correctness of Program Specifications}
An arbitrarily written specification is not necessarily correct. The correctness of specifications must be measured relative to certain criteria~\cite{nimmer2002automatic}. Since we mainly focus on specifications describing the actual behaviors of programs in this work, the correctness of specifications depends on their consistency with program behaviors. A correct specification $s = (\Sigma, f)$ should describe the constraints $f$ that always hold for all program states $\sigma \in \Sigma$ covered, i.e. $f(\sigma)=true$. If any program state $\hat{\sigma} \in \Sigma$ refutes the specification, it becomes a counterexample, and the specification mentioned should be considered incorrect.

\begin{definition}[Correctness of specifications]
A specification $s = (\Sigma, f)$ is considered correct if and only if $\ \forall \sigma \in \Sigma,\ f(\sigma) = true$, denoted as $\mathbf{Cr}(s)=true$. Otherwise, the specification is incorrect, and $\mathbf{Cr}(s)=false$.
\end{definition}
